GNN's Uncertainty Quantification using Self-Distillation

Graph Neural Networks (GNNs) have shown remarkable performance in the healthcare domain. However, what remained challenging is quantifying the predictive uncertainty of GNNs, which is an important aspect of trustworthiness in clinical settings. While Bayesian and ensemble methods can be used to quantify uncertainty, they are computationally expensive. Additionally, the disagreement metric used by ensemble methods to compute uncertainty cannot capture the diversity of models in an ensemble network. In this paper, we propose a novel method, based on knowledge distillation, to quantify GNNs' uncertainty more efficiently and with higher precision. We apply self-distillation, where the same network serves as both the teacher and student models, thereby avoiding the need to train several networks independently. To ensure the impact of self-distillation, we develop an uncertainty metric that captures the diverse nature of the network by assigning different weights to each GNN classifier. We experimentally evaluate the precision, performance, and ability of our approach in distinguishing out-of-distribution data on two graph datasets: MIMIC-IV and Enzymes. The evaluation results demonstrate that the proposed method can effectively capture the predictive uncertainty of the model while having performance similar to that of the MC Dropout and ensemble methods. The code is publicly available at https://github.com/tailabTMU/UQ_GNN.

==> sections/appendices.tex <==
\section{Appendix}\label{sec:appendix}
% \subsection{Models}\label{apd:models}
% We used a different model for each dataset utilized in this study.

% \paragraph{MIMIC-IV Dataset:} For the ensemble model, we trained three identical models but with different random initializations. We followed the same structure provided by \cite{Daneshvar2022Heterogeneous}. Each model consists of three layers of the GraphConv operator~\cite{morris2021weisfeiler} followed by the ReLU activation function. The proposed pooling function of \cite{Daneshvar2022Heterogeneous} was used to aggregate the node-level representations into a single graph-level embedding. Finally, a linear layer is employed for graph classification. We used the soft-voting technique to predict the class in the ensemble. The soft-voting technique computes the mean probability of each class predicted by the classifiers and selects the label with the highest predicted probability. For the self-distillation method, a three-layer GNN is trained. The model structure is similar to the structure used in the ensemble models described above. However, after each graph layer, the same graph pooling layer and linear layer are used to classify the input data. The deepest classifier is used as the reference (and outcome) model for predictions. The model used for the MC Dropout technique is similar to each individual model in the ensemble with an active dropout layer before the classification head.

% \paragraph{Enzymes Dataset:} For the ensemble model, we trained four identical models but with different random initializations. Each model follows the GNN structure provided by~\cite{Dwivedi2023}. To generate node embeddings, the data is passed through an initial transformation comprising a linear layer followed by a dropout layer. These embeddings, in conjunction with each graph's adjacency matrix, are subsequently processed through a four-layer GraphSAGE operator~\cite{NIPS2017_hamilton} employing the ReLU activation function. A max pooling operation is then utilized to aggregate the node-level representations into a single graph-level embedding. Finally, a two-layer multilayer perceptron (MLP) is employed for graph classification. We adopted the GraphSAGE configuration recommended by~\cite{Dwivedi2023}. We used the soft-voting technique to predict the class. For the self-distillation method, a four-layer GNN is trained. The model structure is similar to the structure used in the ensemble models described above. However, after each graph layer, the same graph pooling layer and 2-layer MLP are used to classify the input data. The deepest classifier is used as the reference (and outcome) model for predictions. The MC Dropout technique utilizes the same structure as each individual model in the ensemble with an active dropout layer before the classification head

% \subsection{Additional Results}\label{apd:more_res}
% \subsubsection{Performance and Computational Cost}\label{apd:sub:perf_cost}
% Table~\ref{tab:parameters} shows the number of trainable parameters for each model. The ensemble approach has four and three times the number of parameters of a single model for the enzymes dataset and the MIMIC-IV dataset, respectively, which corresponds to the number of models used in the ensemble. The self-distillation and MC Dropout approaches have a number of parameters comparable to those of the single model. Thus, both methods are more computationally efficient to train. However, during the inference, since 100 samples are drawn from the MC Dropout predictions, i.e., the MC Dropout model runs 100 times, the number of computations would be larger than the self-distillation approach. Therefore, the self-distillation approach is more computationally efficient. This is especially important when deploying models to computationally restricted devices.

% \begin{table}[ht]
%     \centering
%     \caption{Number of trainable parameter of each model.}\label{tab:parameters}
%         \begin{tabular}{|c|c|c|}
%         \hline
%              \textbf{Dataset}&\textbf{Model} & \textbf{No. Params}\\
%             \hline
%              \multirow{4}{*}{Enzymes}&Single Model& 73,082\\
%   &MC Dropout& 73,082\\
%   &Ensemble& 292,328\\
%              &Self-Distillation& 88,748\\
%             \hline
%              \multirow{4}{*}{MIMIC-IV}&Single Model& 142,978\\
%   &MC Dropout& 142,978\\
%   &Ensemble& 428,934\\
%              &Self-Distillation& 144,006\\
%              \hline
%         \end{tabular}
% \end{table}

% We have also included additional results on the performance and calibration error of the approaches in Table~\ref{tab:more_details}. As can be seen, the proposed approach has a similar performance to other approaches, and for each dataset, the trained models have nearly similar calibration errors.

% \begin{table}[ht]
%     \centering
%     \caption{The performance and calibration error of the approaches.}\label{tab:more_details}
%         \begin{tabular}{|c|c|c|c|c|c|}
%         \hline
%              \textbf{Dataset}&\textbf{Model} & \textbf{ROC AUC} 
% & \textbf{MCE}& \textbf{Brier}&\textbf{NLL}\\
% \hline
%   \multirow{3}{*}{\textbf{Enzymes}}&MC Dropout& 0.88 $\pm$ 0.02
% & 0.46 $\pm$ 0.08& 0.53 $\pm$ 0.05&1.63 $\pm$ 0.27\\
%   &Ensemble& 0.89 $\pm$ 0.02
% & 0.40 $\pm$ 0.12& 0.44 $\pm$ 0.05&1.15 $\pm$ 0.18\\
%              &Self-Distillation& 0.87 $\pm$ 0.02
% & 0.42 $\pm$ 10& 0.51 $\pm$ 0.04&1.44 $\pm$ 0.30\\
% \hline
%   \multirow{3}{*}{\textbf{MIMIC-IV}}&MC Dropout& 0.89 $\pm$ 0.01
% & 0.11 $\pm$ 0.02& 0.11 $\pm$ 0.01&0.40 $\pm$ 0.03\\
%   &Ensemble& 0.89 $\pm$ 0.01
% & 0.15 $\pm$ 0.06& 0.12 $\pm$ 0.02&0.44 $\pm$ 0.02\\
%              &Self-Distillation& 0.90 $\pm$ 0.0& 0.14 $\pm$ 0.06& 0.11 $\pm$ 0.01&0.49 $\pm$ 0.10\\
%              \hline
%         \end{tabular}
% \end{table}

% \begin{table*}[ht]
%     \begin{minipage}{0.65\textwidth}
%     \floatconts
%     {tab:more_details}
%     {\caption{The performance and calibration error of the approaches.}}
%     {\resizebox{1\columnwidth}{!}{
%         \begin{tabular}{c|c|c|c|c|c}
%              \textbf{Dataset}&\textbf{Model} & \textbf{ROC AUC} 
% & \textbf{MCE}& \textbf{Brier}&\textbf{NLL}\\
% \hline
%   \multirow{3}{*}{\textbf{Enzymes}}&MC Dropout& 0.88 $\pm$ 0.02
% & 0.46 $\pm$ 0.08& 0.53 $\pm$ 0.05&1.63 $\pm$ 0.27\\
%   &Ensemble& 0.89 $\pm$ 0.02
% & 0.40 $\pm$ 0.12& 0.44 $\pm$ 0.05&1.15 $\pm$ 0.18\\
%              &Self-Distillation& 0.87 $\pm$ 0.02
% & 0.42 $\pm$ 10& 0.51 $\pm$ 0.04&1.44 $\pm$ 0.30\\
% \hline
%   \multirow{3}{*}{\textbf{MIMIC-IV}}&MC Dropout& 0.89 $\pm$ 0.01
% & 0.11 $\pm$ 0.02& 0.11 $\pm$ 0.01&0.40 $\pm$ 0.03\\
%   &Ensemble& 0.89 $\pm$ 0.01
% & 0.15 $\pm$ 0.06& 0.12 $\pm$ 0.02&0.44 $\pm$ 0.02\\
%              &Self-Distillation& 0.90 $\pm$ 0.0& 0.14 $\pm$ 0.06& 0.11 $\pm$ 0.01&0.49 $\pm$ 0.10\\
%         \end{tabular}
%     }}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.3\textwidth}
%     \floatconts
%     {tab:parameters}
%     {\caption{Number of trainable parameter of each model.}}
%     {\resizebox{1\columnwidth}{!}{
%         \begin{tabular}{c|c|c}
%              \textbf{Dataset}&\textbf{Model} & \textbf{No. Params}\\
%             \hline
%              \multirow{4}{*}{Enzymes}&Single Model& 73,082\\
%   &MC Dropout& 73,082\\
%   &Ensemble& 292,328\\
%              &Self-Distillation& 88,748\\
%             \hline
%              \multirow{4}{*}{MIMIC-IV}&Single Model& 142,978\\
%   &MC Dropout& 142,978\\
%   &Ensemble& 428,934\\
%              &Self-Distillation& 144,006\\
%         \end{tabular}
%     }}
%     \end{minipage}
% \end{table*}

% \subsubsection{More Examples from MIMIC-IV Dataset}\label{apd:sub:mimic_eg}
% Table~\ref{tab:sample_test_uncert_2} and~\ref{tab:sample_test_uncert_vals_2} provide an additional example from the MIMIC-IV dataset. The ground-truth label for both patients is "ADT". The shallowest classifier misclassified Patient~1 as "No ADT" indicating that the patient will not be admitted to the hospital. On the other hand, all classifiers labelled Patient~2 as being admitted to the hospital. Since there are discrepancies between the predictions of the models, the metric should exhibit higher uncertainty. As can be seen in Table~\ref{tab:sample_test_uncert_vals_2}, the conventional disagreement metric cannot capture this discrepancy.

% \begin{table}[ht]
% \centering
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \caption{Two samples from the MIMIC-IV dataset with the ground-truth label of "ADT".}
%     \label{tab:sample_test_uncert_2}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{|c|c|c|c|c|}
%         \hline
%         &\multicolumn{2}{c|}{\textbf{Patient 1}}&\multicolumn{2}{c|}{\textbf{Patient 2}}\\ \hline
%         \textbf{Model} & \textbf{No ADT}& \textbf{ADT}& \textbf{No ADT}& \textbf{ADT}\\ \hline
%         Classifier 1 & \textit{65}& 35& 49.83& \textit{50.17}\\ 
%         Classifier 2 & 19.07& \textit{80.93}& 47.20& \textit{52.80}\\ 
%         Ref. Classifier& 0.29& \textit{99.71}& 0.49& \textit{99.51}\\
%         \hline
%     \end{tabular}
%     }
% \end{minipage}%
% \hfill
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \caption{Sample patients from the MIMIC-IV dataset that shows the agreement metric lacks expressivity.}
%     \label{tab:sample_test_uncert_vals_2}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{|c|c|c|}
%         \hline
%         \textbf{Metrics}&\textbf{Patient 1}&\textbf{Patient 2}\\ \hline
%         Disagreement & 3.7809& 3.7809\\ 
%         UC (Linear Weight) & 0.4618& 0.3901\\ 
%         UC (Nonlinear Weight) & 0.5508& 0.3901\\ 
%         UC\textsubscript{norm} (Linear Weight) & 0.2221& 0.1876\\ 
%         UC\textsubscript{norm} (Nonlinear Weight) & 0.2273& 0.1609\\
%         \hline
%     \end{tabular}
%     }
% \end{minipage}
% \end{table}


% \begin{table}[ht]
% \centering
%     \caption{Two samples from the MIMIC-IV dataset with the ground-truth label of "ADT".}\label{tab:sample_test_uncert_2}
%         \begin{tabular}{|c|c|c|c|c|}
%         \hline
%             &\multicolumn{2}{c|}{\textbf{Patient 1}}&\multicolumn{2}{c|}{\textbf{Patient 2}}\\ \hline
%             \textbf{Model} & \textbf{No ADT}& \textbf{ADT}& \textbf{No ADT}& \textbf{ADT}\\ \hline
%             Classifier 1 & \textit{65}& 35& 49.83& \textit{50.17}\\ 
%             Classifier 2 & 19.07& \textit{80.93}& 47.20& \textit{52.80}\\ 
%             Ref. Classifier& 0.29& \textit{99.71}& 0.49& \textit{99.51}\\
%             \hline
%         \end{tabular}
% \end{table}

% \begin{table}[ht]
% \centering
%     \caption{Sample patients from the MIMIC-IV dataset that shows the agreement metric lacks expressivity.}\label{tab:sample_test_uncert_vals_2}
%         \begin{tabular}{|c|c|c|}
%         \hline
%             \textbf{Metrics}&\textbf{Patient 1}&\textbf{Patient 2}\\ \hline
%             Disagreement & 3.7809& 3.7809\\ 
%             UC (Linear Weight) & 0.4618& 0.3901\\ 
%             UC (Nonlinear Weight) & 0.5508& 0.3901\\ 
%             UC\textsubscript{norm} (Linear Weight) & 0.2221& 0.1876\\ 
%             UC\textsubscript{norm} (Nonlinear Weight) & 0.2273& 0.1609\\
%             \hline
%         \end{tabular}
% \end{table}

% \subsection{Variability of Imitation Parameter}\label{apd:abl}
% We conducted a limited ablation study on the impact of different values of imitation parameter, $\alpha$, in the loss function, on the proposed uncertainty metric. We trained the Self-Distillation approach each time with a different value of $\alpha$ on the Enzymes dataset. The results are shown in Table~\ref{tab:alpha_abl}. When starting from a small imitation parameter, i.e., the student is trying not to be too similar to the teacher, the mean uncertainty is higher. It starts to decrease as it gets closer to 0.9. This indicates less discrepancy between student classifiers and the teacher model. However, as we get closer to the upper bound, the model will be at risk of overfitting to the teacher predictions. Additionally, values below 0.5 might cause the student models to not properly mimic the teacher model. In our experiments, we chose 0.6 for the imitation parameter. The results demonstrate that 0.6 is a valid option as the student predictions are neither too different from nor too similar to the teacher model. However, a more in-depth analysis of hyperparameters is crucial.

% \begin{table}[ht]
% \centering
%     \caption{Impact of different values of $\alpha$ on mean uncertainty metric.}\label{tab:alpha_abl}
%         \begin{tabular}{|c|c|c|}
%         \hline
%             \textbf{$\alpha$}&\textbf{Mean $UC_{linear}$}&\textbf{Mean $UC_{nonlinear}$}\\ \hline
%             0.1& 0.34& 0.40\\ 
%             0.4& 0.21& 0.25\\ 
%             0.6& 0.16& 0.19\\ 
%             0.8& 0.12& 0.14\\
%             \hline
%         \end{tabular}
% \end{table}
